Harvesting Paragraph-Level Question-Answer Pairs from Wikipedia

We study the task of generating from Wikipedia articles question-answer pairs that cover content beyond a single sentence. We propose a neural network approach that incorporates coreference knowledge via a novel gating mechanism. Compared to models that only take into account sentence-level information (Heilman and Smith, 2010; Du et al., 2017; Zhou et al., 2017), we find that the linguistic knowledge introduced by the coreference representation aids question generation significantly, producing models that outperform the current state-of-the-art. We apply our system (composed of an answer span extraction system and the passage-level QG system) to the 10,000 top-ranking Wikipedia articles and create a corpus of over one million question-answer pairs. We also provide a qualitative analysis for this large-scale generated corpus from Wikipedia.

==> acl17bibfile <==
@InProceedings{rajpurkar2016squad,
  author    = {Rajpurkar, Pranav  and  Zhang, Jian  and  Lopyrev, Konstantin  and  Liang, Percy},
  title     = {SQuAD: 100,000+ Questions for Machine Comprehension of Text},
  booktitle = {Proceedings of the 2016 Conference on Empirical Methods in Natural Language Processing (EMNLP)},
  month     = {November},
  year      = {2016},
  address   = {Austin, Texas},
  publisher = {Association for Computational Linguistics},
  pages     = {2383--2392},
  url       = {https://aclweb.org/anthology/D16-1264}
}


@InProceedings{heilman2010good,
  author    = {Heilman, Michael  and  Smith, Noah A.},
  title     = {Good Question! Statistical Ranking for Question Generation},
  booktitle = {Human Language Technologies: The 2010 Annual Conference of the North American Chapter of the Association for Computational Linguistics},
  month     = {June},
  year      = {2010},
  address   = {Los Angeles, California},
  publisher = {Association for Computational Linguistics},
  pages     = {609--617},
  url       = {http://www.aclweb.org/anthology/N10-1086}
}


@InProceedings{papineni2002bleu,
  author    = {Kishore Papineni  and  Salim Roukos  and  Todd Ward  and  Wei-Jing Zhu},
  title     = {Bleu: a Method for Automatic Evaluation of Machine Translation},
  booktitle = {Proceedings of 40th Annual Meeting of the Association for Computational Linguistics},
  month     = {July},
  year      = {2002},
  address   = {Philadelphia, Pennsylvania, USA},
  publisher = {Association for Computational Linguistics},
  pages     = {311--318},
  url       = {http://www.aclweb.org/anthology/P02-1040},
  doi       = {10.3115/1073083.1073135}
}


@InProceedings{2014meteor,
  author    = {Denkowski, Michael  and  Lavie, Alon},
  title     = {Meteor Universal: Language Specific Translation Evaluation for Any Target Language},
  booktitle = {Proceedings of the Ninth Workshop on Statistical Machine Translation},
  month     = {June},
  year      = {2014},
  address   = {Baltimore, Maryland, USA},
  publisher = {Association for Computational Linguistics},
  pages     = {376--380},
  url       = {http://www.aclweb.org/anthology/W14-3348}
}



@inproceedings{lin2004rouge,
  author    = {Lin, Chin-Yew},
  title     = {ROUGE: A Package for Automatic Evaluation of Summaries},
  booktitle = {Text Summarization Branches Out: Proceedings of the ACL-04 Workshop},
  editor = {Marie-Francine Moens, Stan Szpakowicz},
  year      = 2004,
  month     = {July},
  address   = {Barcelona, Spain},
  publisher = {Association for Computational Linguistics},
  pages     = {74--81},
  url       = {http://aclweb.org/anthology/W/W04/W04-1013.pdf}
}

@inproceedings{levenshtein1966binary,
  title={Binary codes capable of correcting deletions, insertions and reversals},
  author={Levenshtein, Vladimir I},
  booktitle={Soviet physics doklady},
  volume={10},
  pages={707},
  year={1966}
}

@inproceedings{vanderwende2008importance,
  title={The importance of being important: Question generation},
  author={Vanderwende, Lucy},
  booktitle={Proceedings of the 1st Workshop on the Question Generation Shared Task Evaluation Challenge, Arlington, VA},
  year={2008}
}

@article{chen2015microsoft,
  title={Microsoft COCO captions: Data collection and evaluation server},
  author={Chen, Xinlei and Fang, Hao and Lin, Tsung-Yi and Vedantam, Ramakrishna and Gupta, Saurabh and Doll{\'a}r, Piotr and Zitnick, C Lawrence},
  journal={arXiv preprint arXiv:1504.00325},
  year={2015}
}


@inproceedings{mitkov2003computer,
  author = {Mitkov, Ruslan  and  Ha, Le An},
  title  = {Computer-Aided Generation of Multiple-Choice Tests},
  booktitle = {Proceedings of the HLT-NAACL 03 Workshop on Building Educational Applications Using Natural Language Processing},
  editor = {Jill Burstein and Claudia Leacock},
  url    = {http://www.aclweb.org/anthology/W03-0203.pdf},
  year   = 2003,
  pages  = {17--22}
}


@inproceedings{rus2010first,
 author = {Rus, Vasile and Wyse, Brendan and Piwek, Paul and Lintean, Mihai and Stoyanchev, Svetlana and Moldovan, Cristian},
 title = {The First Question Generation Shared Task Evaluation Challenge},
 booktitle = {Proceedings of the 6th International Natural Language Generation Conference},
 year = {2010},
 pages = {251--257},
 url = {http://dl.acm.org/citation.cfm?id=1873738.1873777},
 publisher = {Association for Computational Linguistics},
 address = {Stroudsburg, PA, USA},
} 

@book{chomsky1971conditions,
  title={Conditions on transformations},
  author={Chomsky, Noam},
  year={1971},
  publisher={Indiana University, Linguistics Club}
}

@inproceedings{bahdanau2014neural,
  title={Neural machine translation by jointly learning to align and translate},
  author={Bahdanau, Dzmitry and Cho, Kyunghyun and Bengio, Yoshua},
  booktitle={International Conference on Learning Representations Workshop (ICLR)},
  year={2015}
}

@inproceedings{koehn2007moses,
 author = {Koehn, Philipp and Hoang, Hieu and Birch, Alexandra and Callison-Burch, Chris and Federico, Marcello and Bertoldi, Nicola and Cowan, Brooke and Shen, Wade and Moran, Christine and Zens, Richard and Dyer, Chris and Bojar, Ond\v{r}ej and Constantin, Alexandra and Herbst, Evan},
 title = {Moses: Open Source Toolkit for Statistical Machine Translation},
 booktitle = {Proceedings of the 45th Annual Meeting of the ACL on Interactive Poster and Demonstration Sessions},
 year = {2007},
 pages = {177--180},
 url = {http://dl.acm.org/citation.cfm?id=1557769.1557821},
 publisher = {Association for Computational Linguistics},
 address = {Stroudsburg, PA, USA},
} 

@InProceedings{luong2015effective,
  author    = {Luong, Thang  and  Pham, Hieu  and  Manning, Christopher D.},
  title     = {Effective Approaches to Attention-based Neural Machine Translation},
  booktitle = {Proceedings of the 2015 Conference on Empirical Methods in Natural Language Processing},
  month     = {September},
  year      = {2015},
  address   = {Lisbon, Portugal},
  publisher = {Association for Computational Linguistics},
  pages     = {1412--1421},
  url       = {http://aclweb.org/anthology/D15-1166}
}


@InProceedings{serban2016factoid30m,
  author    = {Serban, Iulian Vlad  and  Garc\'{i}a-Dur\'{a}n, Alberto  and  Gulcehre, Caglar  and  Ahn, Sungjin  and  Chandar, Sarath  and  Courville, Aaron  and  Bengio, Yoshua},
  title     = {Generating Factoid Questions With Recurrent Neural Networks: The 30M Factoid Question-Answer Corpus},
  booktitle = {Proceedings of the 54th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  month     = {August},
  year      = {2016},
  address   = {Berlin, Germany},
  publisher = {Association for Computational Linguistics},
  pages     = {588--598},
  url       = {http://www.aclweb.org/anthology/P16-1056}
}

@InProceedings{nasrin2016vqg,
  author    = {Mostafazadeh, Nasrin  and  Misra, Ishan  and  Devlin, Jacob  and  Mitchell, Margaret  and  He, Xiaodong  and  Vanderwende, Lucy},
  title     = {Generating Natural Questions About an Image},
  booktitle = {Proceedings of the 54th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  month     = {August},
  year      = {2016},
  address   = {Berlin, Germany},
  publisher = {Association for Computational Linguistics},
  pages     = {1802--1813},
  url       = {http://www.aclweb.org/anthology/P16-1170}
}


@InProceedings{rush2015namas,
  author    = {Rush, Alexander M.  and  Chopra, Sumit  and  Weston, Jason},
  title     = {A Neural Attention Model for Abstractive Sentence Summarization},
  booktitle = {Proceedings of the 2015 Conference on Empirical Methods in Natural Language Processing},
  month     = {September},
  year      = {2015},
  address   = {Lisbon, Portugal},
  publisher = {Association for Computational Linguistics},
  pages     = {379--389},
  url       = {http://aclweb.org/anthology/D15-1044}
}


@ARTICLE{2017opennmt,
         author = { {Klein}, Guillaume and {Kim}, Yoon and {Deng}, Yuntian 
                    and {Senellart}, Jean and {Rush}, Alexander M.},
         title = {OpenNMT: Open-Source Toolkit 
                   for Neural Machine Translation},
         year  = {2017},
         journal = {ArXiv e-prints},
         eprint = {1701.02810} }
         
@inproceedings{hermann2015teaching,
  title={Teaching machines to read and comprehend},
  author={Hermann, Karl Moritz and Kocisky, Tomas and Grefenstette, Edward and Espeholt, Lasse and Kay, Will and Suleyman, Mustafa and Blunsom, Phil},
  booktitle={Advances in Neural Information Processing Systems (NIPS)},
  pages={1693--1701},
  year={2015}
}

@InProceedings{weston2015towards,
  author={Weston, Jason and Bordes, Antoine and Chopra, Sumit and Rush, Alexander M and van Merri{\"e}nboer, Bart and Joulin, Armand and Mikolov, Tomas},
  title={Towards ai-complete question answering: A set of prerequisite toy tasks},
  booktitle={International Conference on Learning Representations Workshop (ICLR)},
  year={2016}
}

@InProceedings{danqi2016exam,
  author    = {Chen, Danqi  and  Bolton, Jason  and  Manning, Christopher D.},
  title     = {A Thorough Examination of the CNN/Daily Mail Reading Comprehension Task},
  booktitle = {Proceedings of the 54th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  month     = {August},
  year      = {2016},
  address   = {Berlin, Germany},
  publisher = {Association for Computational Linguistics},
  pages     = {2358--2367},
  url       = {http://www.aclweb.org/anthology/P16-1223}
}

@InProceedings{richardson2013mctest,
  author    = {Richardson, Matthew  and  Burges, Christopher J.C.  and  Renshaw, Erin},
  title     = {{MCTest}: A Challenge Dataset for the Open-Domain Machine Comprehension of Text},
  booktitle = {Proceedings of the 2013 Conference on Empirical Methods in Natural Language Processing},
  month     = {October},
  year      = {2013},
  address   = {Seattle, Washington, USA},
  publisher = {Association for Computational Linguistics},
  pages     = {193--203},
  url       = {http://www.aclweb.org/anthology/D13-1020}
}

@inproceedings{sutskever2014sequence,
  title={Sequence to sequence learning with neural networks},
  author={Sutskever, Ilya and Vinyals, Oriol and Le, Quoc V},
  booktitle={Advances in neural information processing systems (NIPS)},
  pages={3104--3112},
  year={2014}
}
@inproceedings{xu2015show,
  title={Show, Attend and Tell: Neural Image Caption Generation with Visual Attention.},
  author={Xu, Kelvin and Ba, Jimmy and Kiros, Ryan and Cho, Kyunghyun and Courville, Aaron C and Salakhutdinov, Ruslan and Zemel, Richard S and Bengio, Yoshua},
  booktitle={ICML},
  volume={14},
  pages={77--81},
  year={2015}
}


@inproceedings{mostow2009generating,
  title={Generating Instruction Automatically for the Reading Strategy of Self-Questioning.},
  author={Mostow, Jack and Chen, Wei},
  booktitle={Proceedings of the 2nd Workshop on Question Generation (AIED 2009)},
  pages={465--472},
  year={2009}
}

@InProceedings{mazidi2014linguistic,
  author    = {Mazidi, Karen  and  Nielsen, Rodney D.},
  title     = {Linguistic Considerations in Automatic Question Generation},
  booktitle = {Proceedings of the 52nd Annual Meeting of the Association for Computational Linguistics (Volume 2: Short Papers)},
  month     = {June},
  year      = {2014},
  address   = {Baltimore, Maryland},
  publisher = {Association for Computational Linguistics},
  pages     = {321--326},
  url       = {http://www.aclweb.org/anthology/P14-2053}
}


@InProceedings{lindberg2013online,
  author    = {Lindberg, David  and  Popowich, Fred  and  Nesbit, John  and  Winne, Phil},
  title     = {Generating Natural Language Questions to Support Learning On-Line},
  booktitle = {Proceedings of the 14th European Workshop on Natural Language Generation},
  month     = {August},
  year      = {2013},
  address   = {Sofia, Bulgaria},
  publisher = {Association for Computational Linguistics},
  pages     = {105--114},
  url       = {http://www.aclweb.org/anthology/W13-2114}
}

@InProceedings{labutov2015deep,
  author    = {Labutov, Igor  and  Basu, Sumit  and  Vanderwende, Lucy},
  title     = {Deep Questions without Deep Understanding},
  booktitle = {Proceedings of the 53rd Annual Meeting of the Association for Computational Linguistics and the 7th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)},
  month     = {July},
  year      = {2015},
  address   = {Beijing, China},
  publisher = {Association for Computational Linguistics},
  pages     = {889--898},
  url       = {http://www.aclweb.org/anthology/P15-1086}
}

@book{manning2008introduction,
 author = {Manning, Christopher D. and Raghavan, Prabhakar and Sch\"{u}tze, Hinrich},
 title = {Introduction to Information Retrieval},
 year = {2008},
 isbn = {0521865719, 9780521865715},
 publisher = {Cambridge University Press},
 address = {New York, NY, USA},
}

@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press}
}

@InProceedings{luong2015addressing,
  author    = {Luong, Thang  and  Sutskever, Ilya  and  Le, Quoc  and  Vinyals, Oriol  and  Zaremba, Wojciech},
  title     = {Addressing the Rare Word Problem in Neural Machine Translation},
  booktitle = {Proceedings of the 53rd Annual Meeting of the Association for Computational Linguistics and the 7th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)},
  month     = {July},
  year      = {2015},
  address   = {Beijing, China},
  publisher = {Association for Computational Linguistics},
  pages     = {11--19},
  url       = {http://www.aclweb.org/anthology/P15-1002}
}

@InProceedings{pennington2014glove,
  author    = {Pennington, Jeffrey  and  Socher, Richard  and  Manning, Christopher},
  title     = {Glove: Global Vectors for Word Representation},
  booktitle = {Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing (EMNLP)},
  month     = {October},
  year      = {2014},
  address   = {Doha, Qatar},
  publisher = {Association for Computational Linguistics},
  pages     = {1532--1543},
  url       = {http://www.aclweb.org/anthology/D14-1162}
}


@InProceedings{manning2014corenlp,
  author    = {Manning, Christopher  and  Surdeanu, Mihai  and  Bauer, John  and  F., Jenny  and  B., Steven  and  M., David},
  title     = {The Stanford CoreNLP Natural Language Processing Toolkit},
  booktitle = {Proceedings of 52nd Annual Meeting of the Association for Computational Linguistics: System Demonstrations},
  month     = {June},
  year      = {2014},
  address   = {Baltimore, Maryland},
  publisher = {Association for Computational Linguistics},
  pages     = {55--60},
  url       = {http://www.aclweb.org/anthology/P14-5010}
}

@InProceedings{KenLM2015,
  author    = {Heafield, Kenneth  and  Pouzyrevsky, Ivan  and  Clark, Jonathan H.  and  Koehn, Philipp},
  title     = {Scalable Modified Kneser-Ney Language Model Estimation},
  booktitle = {Proceedings of the 51st Annual Meeting of the Association for Computational Linguistics (Volume 2: Short Papers)},
  month     = {August},
  year      = {2013},
  address   = {Sofia, Bulgaria},
  publisher = {Association for Computational Linguistics},
  pages     = {690--696},
  url       = {http://www.aclweb.org/anthology/P13-2121}
}

@article{nguyen2016msmarco,
  title={MS MARCO: A Human Generated MAchine Reading COmprehension Dataset},
  author={Nguyen, Tri and Rosenberg, Mir and Song, Xia and Gao, Jianfeng and Tiwary, Saurabh and Majumder, Rangan and Deng, Li},
  journal={arXiv preprint arXiv:1611.09268},
  year={2016}
}

@article{Weizenbaum1966eliza,
 author = {Weizenbaum, Joseph},
 title = {ELIZA\&Mdash;a Computer Program for the Study of Natural Language Communication Between Man and Machine},
 journal = {Commun. ACM},
 issue_date = {Jan. 1966},
 volume = {9},
 number = {1},
 month = jan,
 year = {1966},
 issn = {0001-0782},
 pages = {36--45},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/365153.365168},
 doi = {10.1145/365153.365168},
 acmid = {365168},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@article{parry1971colby,
  author    = {Kenneth Mark Colby and
               Sylvia Weber and
               Franklin Dennis Hilf},
  title     = {Artificial Paranoia},
  journal   = {Artificial Intelligence},
  volume    = {2},
  number    = {1},
  pages     = {1--25},
  year      = {1971},
  url       = {http://dx.doi.org/10.1016/0004-3702(71)90002-6},
  doi       = {10.1016/0004-3702(71)90002-6},
}

@article{surveyhumanrobot03,
  author    = {Terrence Fong and
               Illah R. Nourbakhsh and
               Kerstin Dautenhahn},
  title     = {A survey of socially interactive robots},
  journal   = {Robotics and Autonomous Systems},
  volume    = {42},
  number    = {3-4},
  pages     = {143--166},
  year      = {2003},
  url       = {http://dx.doi.org/10.1016/S0921-8890(02)00372-X},
  doi       = {10.1016/S0921-8890(02)00372-X},
}

@article{zaremba2014recurrent,
  title={Recurrent neural network regularization},
  author={Zaremba, Wojciech and Sutskever, Ilya and Vinyals, Oriol},
  journal={arXiv preprint arXiv:1409.2329},
  year={2014}
}

@InProceedings{chopra2016abstractive,
  author    = {Chopra, Sumit  and  Auli, Michael  and  Rush, Alexander M.},
  title     = {Abstractive Sentence Summarization with Attentive Recurrent Neural Networks},
  booktitle = {Proceedings of the 2016 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
  month     = {June},
  year      = {2016},
  address   = {San Diego, California},
  publisher = {Association for Computational Linguistics},
  pages     = {93--98},
  url       = {http://www.aclweb.org/anthology/N16-1012}
}


@InProceedings{cho2014phrase,
  author    = {Cho, Kyunghyun  and  van Merrienboer, Bart  and  Gulcehre, Caglar  and  Bahdanau, Dzmitry  and  Bougares, Fethi  and  Schwenk, Holger  and  Bengio, Yoshua},
  title     = {Learning Phrase Representations using RNN Encoder--Decoder for Statistical Machine Translation},
  booktitle = {Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing (EMNLP)},
  month     = {October},
  year      = {2014},
  address   = {Doha, Qatar},
  publisher = {Association for Computational Linguistics},
  pages     = {1724--1734},
  url       = {http://www.aclweb.org/anthology/D14-1179}
}

@inproceedings{robertson1994bm25,
 author = {Robertson, Stephen E. and Walker, Steve},
 title = {Some Simple Effective Approximations to the 2-Poisson Model for Probabilistic Weighted Retrieval},
 booktitle = {Proceedings of the 17th Annual International ACM SIGIR Conference on Research and Development in Information Retrieval},
 series = {SIGIR '94},
 year = {1994},
 pages = {232--241},
 numpages = {10},
 url = {http://dl.acm.org/citation.cfm?id=188490.188561},
 publisher = {Springer-Verlag New York, Inc.},
 address = {New York, NY, USA},
} 

@InProceedings{iyer2016code,
  author    = {Iyer, Srinivasan  and  Konstas, Ioannis  and  Cheung, Alvin  and  Zettlemoyer, Luke},
  title     = {Summarizing Source Code using a Neural Attention Model},
  booktitle = {Proceedings of the 54th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  month     = {August},
  year      = {2016},
  address   = {Berlin, Germany},
  publisher = {Association for Computational Linguistics},
  pages     = {2073--2083},
  url       = {http://www.aclweb.org/anthology/P16-1195}
}


